RP-DNN: A Tweet level propagation context based deep neural networks for early rumor detection in Social Media

Early rumor detection (ERD) on social media platform is very challenging when limited, incomplete and noisy information is available. Most of the existing methods have largely worked on event-level detection that requires the collection of posts relevant to a specific event and relied only on user-generated content. They are not appropriate to detect rumor sources in the very early stages, before an event unfolds and becomes widespread. In this paper, we address the task of ERD at the message level. We present a novel hybrid neural network architecture, which combines a task-specific character-based bidirectional language model and stacked Long Short-Term Memory (LSTM) networks to represent textual contents and social-temporal contexts of input source tweets, for modelling propagation patterns of rumors in the early stages of their development. We apply multi-layered attention models to jointly learn attentive context embeddings over multiple context inputs. Our experiments employ a stringent leave-one-out cross-validation (LOO-CV) evaluation setup on seven publicly available real-life rumor event data sets. Our models achieve state-of-the-art(SoA) performance for detecting unseen rumors on large augmented data which covers more than 12 events and 2,967 rumors. An ablation study is conducted to understand the relative contribution of each component of our proposed model.

==> sections/appendices.tex <==
\section{Appendices}\label{appendices}

Table \ref{tab:appendix_globalnorm} presents the global means and standard deviation computed from whole training set and used to normalise feature representations of context metadata.

\begin{table*}[t]
{\footnotesize\begin{tabular}{
            p{\dimexpr 0.12 \linewidth-2.4\tabcolsep}
				p{\dimexpr 0.25 \linewidth-2.8\tabcolsep}
				p{\dimexpr 0.15 \linewidth-2.6\tabcolsep}
				p{\dimexpr 0.15 \linewidth-2.6\tabcolsep}
				p{\dimexpr 0.15 \linewidth-3.0\tabcolsep}
				p{\dimexpr 0.15 \linewidth-3.0\tabcolsep}}
\multirow{1}{*}{\bf } & \bf NFs & \bf global mean & \bf global std. & \bf global max & \bf global min \\ \hline
\multirow{4}{*}{user features} & \# of posts & 53687.5965 & 127457.9930 & 4420429 & 1 \\	
    & listed count & 102.4828 & 1228.3984 & 199211 & 0 \\
    & followers & 7174.8032 & 233721.4625 & 42822106 & 0 \\
    & followings & 1679.2319 & 8920.4870 & 1602789 & 0 \\
    & follow ratio & 163.1336 & 31374.2225 & 9918751.75 & 0\\ 
    & follow ratio (v2) & 0.4722 & 0.2282 & 1 & 0 \\ 
    & \# of user favourites & 18493.6203 & 49741.6807 & 2419251 & 0 \\
    & account age & 1197.2359 & 686.5547 & 3611 & 1 \\
    & is verified & 0.0269 & 0.1618 & 1 & 0 \\
    & engagement scr & 82.5727 & 534.0954 & 164474.5 & 0.0005 \\
    & following rate & 3.7328 & 32.6771 & 6207.4 & 0 \\
    & favourites scr & 38.3545 & 407.0863 & 85537 & 0 \\ 
    & is GEO enabled & 0.5282 & 0.4992 & 1 & 0 \\ 
    & description length & 11.7235 & 8.7322 & 64 & 0 \\
    & user profile name length & 11.6878 & 5.5836 & 50 & 0 \\
    & is source user & 0.0098 & 0.0987 & 1 & 0 \\ \hline
\multirow{3}{*}{tweet features} & \# of retweets & 263.1094 & 1040.1257 & 77459 & 0 \\
    & \# of favorites & 0.3600 & 36.3189 & 22836 & 0 \\
    & has question & 0.0579 & 0.2336 & 1 & 0 \\
    & is duplicated & 0.0011 & 0.0324 & 1 & 0 \\
    & has image & 0.8762 & 0.3294 & 1 & 0 \\
    & has URL & 0.3083 & 0.4618 & 1 & 0 \\
    & \# of URL & 0.31187853 & 0.4712 & 5 & 0 \\
    & has native media & 0.1679 & 0.3738 & 1 & 0 \\
    & context content length & 15.8925 & 5.5011 & 47 & 0 \\
    & response time decay (mins.) & 1664.1876 & 42754.3823 & 3152616.7667 & 0 \\
    % & context type  & 0.2117 & 0.4085 & 1 & 0 \\
    & has user profile desc  & 0.8529 & 0.3542 & 1 & 0 \\\hline
\end{tabular}}{\caption{Statistics of global Mean-variance in whole training set}
      \label{tab:appendix_globalnorm}}
\end{table*}


==> sections/dataset.tex <==
\section{Data Set} \label{dataset}
% Statitics of dataset in the experiment: training set, heldout set, test set, 

% statistics of each hold-out event dataset in terms of # of rumours, # of non-rumours, # of retweets, # of replies, Avg. # of retweets per hold-out event dataset, Avg. # of replies per hold-out event dataset, Max # of retweets, Max # of replies, Min # retweets, Min # of replies, Median # of retweets, Median # of replies, etc.

% TODO: re-emphasis the data scarcity challenging in ERD and explain why some public dataset \cite{ma2016detecting} cannot be used in our task.

We experiment with two data sets: PHEME 6392078 datasets and Twitter 15/16 dataset (\textcolor{red}{TODO: update with latest train, hold-out and test dataset. We will list statistics of all (>10) the event dataset used in train set and the 7 LOOCV dataset}).
\begin{enumerate}[noitemsep]
	\item \textbf{Aug-rnr} \citelanguageresource{han2019neural}: This is an augmented version of PHEME(6392078). It contains rumour and non-rumour source tweets and their contexts (i.e., replies and retweets) associated with six real-world breaking news events. Source tweets are labelled with weak supervision. 
	\item \textbf{Twitter15 and Twitter16} \cite{ma2017detect}: These data sets consist of rumor and non-rumor source tweets and their contexts. Contexts for each source tweet are provided in the form of propagation trees. Source tweets are annotated with one of four categories: non-rumor, false rumor, true rumor and unverified rumor. These are used as test sets during evaluation.
	\item \textbf{PHEME(6392078) \cite{kochkina2018all}}  This data consists of manually labeled rumors and non-rumors for 9 events. It is used as test sets during evaluation.
\end{enumerate}	

Statistics of our training and test sets are presented in Table \ref{tab:testset_statistics}.

\begin{table}[t!]
	\caption{Statistics of test set with balanced rumor and non-rumor source tweets}
	\begin{center}
		\footnotesize
		\begin{tabular}{p{\dimexpr 0.236 \linewidth-2.4\tabcolsep}
				p{\dimexpr 0.21\linewidth-2.8\tabcolsep}
				p{\dimexpr 0.2\linewidth-2.6\tabcolsep}
			\bf Hold-out Event  & \bf \# of rumor tweets &\bf \# of non-rumor tweets  \\ \hline
			bostonbombings        	& 323  & 323 \\
			charliehebdo      	& 458 & 458 \\
           ferguson      	& 284 & 284 \\
			germanwings & 231 & 231 \\
          ottawashooting & 420 & 420 \\
           sydneysiege & 522 & 522 \\
		\end{tabular}
		\label{tab:testset_statistics}
	\end{center}
\end{table}



%\begin{table}[t!]
%	\caption{Statitics of dataset}
%	\begin{center}
%		\footnotesize
%		\begin{tabular}{p{\dimexpr 0.236 \linewidth-2.4\tabcolsep}
%				p{\dimexpr 0.21\linewidth-2.8\tabcolsep}
%				p{\dimexpr 0.2\linewidth-2.6\tabcolsep}
%			
%			\bf Event  & \bf \# of English tweets &\bf # of unique English tweets\(after preprocessing\)  \\ \hline
			
%			Christchurch shooting        	& 622,384 & 460,477 \\
%			Manchester arena bombing      	& 917,749 & 890,251 \\
%			
%		\end{tabular}
%		\label{tab:event1216}
%	\end{center}
%\end{table}


==> sections/method_data_processing.tex <==
\section{Data processing}\label{method_dataprocessing}

We follow a simple pre-processing practice proposed in \cite{alhuzali2018ubc}. All tweets are lowercased, and URLs and user mentions are removed. Embedded links can be considered as critical metadata for rumor detection as they may help to identify sources of potential rumours. However, external information except textual information is not exploited for obtaining semantic and syntactic embeddings via ELMo. Tweets with a minimum of 4 tokens are considered as tweets which lack enough textual features are generally unremarkable and add noise to data~\citep{Ifrim2014Event}.


